$M^3-Verse$: A "Spot the Difference" Challenge for Large Multimodal Models

Modern Large Multimodal Models (LMMs) have demonstrated extraordinary ability in static image and single-state spatial-temporal understanding. However, their capacity to comprehend the dynamic changes of objects within a shared spatial context between two distinct video observations, remains largely unexplored. This ability to reason about transformations within a consistent environment is particularly crucial for advancements in the field of spatial intelligence. In this paper, we introduce $M^3-Verse$, a Multi-Modal, Multi-State, Multi-Dimensional benchmark, to formally evaluate this capability. It is built upon paired videos that provide multi-perspective observations of an indoor scene before and after a state change. The benchmark contains a total of 270 scenes and 2,932 questions, which are categorized into over 50 subtasks that probe 4 core capabilities. We evaluate 16 state-of-the-art LMMs and observe their limitations in tracking state transitions. To address these challenges, we further propose a simple yet effective baseline that achieves significant performance improvements in multi-state perception. $M^3-Verse$ thus provides a challenging new testbed to catalyze the development of next-generation models with a more holistic understanding of our dynamic visual world. You can get the construction pipeline from https://github.com/Wal-K-aWay/M3-Verse_pipeline and full benchmark data from https://www.modelscope.cn/datasets/WalKaWay/M3-Verse.

==> sec/5_analysis_old.tex <==
\section{Diagnostic Analysis: Isolating the Bottleneck}

\begin{figure*}
  \centering
  \begin{subfigure}{0.45\linewidth}
    \centerline{\includegraphics[width=\textwidth]{imgs/baseline_overall_improve.pdf}}
    \caption{Performance comparison measured by Overall Score. Left: End-to-End performance, Right: Text-Oracle performance.}
    \label{fig:baseline overall}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.5\linewidth}
    \centerline{\includegraphics[width=\textwidth]{imgs/sankey_text_oracle.pdf}}
    \caption{Performance in Inter-state subset. Blue: correct samples, Orange: incorrect samples.}
    \label{fig:inter}
  \end{subfigure}
  \caption{Isolating the reasoning bottleneck via \textbf{Text-Oracle diagnosis}, measured by (a) Overall Score and (b) Inter-state Average.}
  \label{fig:baseline}
\end{figure*}

\subsection{Text-Oracle Probe}
% To address the inherent challenges LMMs face in processing long-form videos and tracking temporal state changes, we introduce the \textbf{Text-Oracle Pipeline}. Instead of end-to-end video processing, this method transforms the multimodal reasoning problem into a text-based task through a three-stage process.

Given the poor performance of SOTA models, a critical question arises: Are these failures caused by the LLM's inability to perform logical reasoning, or by the vision encoder's failure to capture fine-grained state changes? To decouple these factors and answer this question, we designed a diagnostic experimental setup, which we term the \textbf{Text-Oracle Probe}. This probe artificially bypasses the dynamic visual-language alignment phase by explicitly translating the visual stream into text before reasoning. The probe operates through a 3-stage process:

\begin{enumerate}
    \item \textbf{Video Segmentation and Dense Captioning.} A given video is first partitioned into a sequence of non-overlapping temporal clips. An LMM is then applied to generate a detailed textual description of each clip along with its start time and end time. This converts the visual stream into a set of captions, each associated with a specific time interval.
    \item \textbf{Cohesive Summary Generation.} The sequence of time-coded captions is then consolidated by LLM or LMM, into a single, cohesive narrative summary.
    \item \textbf{Text-based Question Answering.} Finally, the generated summaries of two videos are concatenated with the question. An LLM or LMM is applied to answer the question based on text-only descriptions of the videos.
\end{enumerate}

\subsection{Diagnostic Results and Analysis}
We conducted this diagnostic experiment on InternVL3.5-Instruct~\cite{InternVL3.5} and Qwen3-VL-Instruct~\cite{qwen3-vl} at 4B and 8B scale. The results, presented in Fig~\ref{fig:baseline}, demonstrate a stark contrast between standard end-to-end performance and the text-oracle setting. Crucially, this significant gap exposes exactly where current LMMs fail when handling dynamic visual contexts.

\noindent\textbf{Performance Discrepancy under the Text-Oracle Setting.}
% Here we utilize the LMM for all stages: generating clip captioning, summarization and eventually answering. The hierarchical captioning method consistently and significantly outperforms the standard direct video QA method across most tested models. For instance, InternVL3.5-8B-Instruct~\cite{InternVL3.5} sees its overall accuracy jump by over 7 absolute points. Similarly, Qwen3-VL-8B-Instruct~\cite{qwen3-vl} achieves an improvement of more than 4 absolute points compared to its standard counterpart. This shows that structuring the reasoning process yields a more effective and robust understanding.
Here, we utilize the LMM to execute all stages of the probe: generating clip captions, summarizing them, and eventually answering the question based on the text. The results reveal that this text-oracle setup consistently and significantly yields higher performance than the standard direct video QA baseline across most tested models. For instance, InternVL3.5-8B-Instruct~\cite{InternVL3.5} sees its overall accuracy jump by over 7 absolute points when evaluated through this text-only intermediate route. Similarly, Qwen3-VL-8B-Instruct~\cite{qwen3-vl} achieves an improvement of more than 4 absolute points compared to its standard end-to-end counterpart. This substantial discrepancy demonstrates that when visual events are explicitly structured and serialized into text, the underlying models are far more capable of robustly answering the questions. This suggests that the primary bottleneck in the standard end-to-end process lies in the direct processing and alignment of raw visual features, rather than an inherent lack of understanding or logic within the models themselves.

% \noindent\textbf{Dramatically Enhanced Inter-State Reasoning.}
% The most pronounced improvements are observed in the \textbf{`inter-state'} evaluation, which is the core challenge of our benchmark. As shown in Fig~\ref{fig:inter}, for InternVL3.5-8B-Instruct~\cite{InternVL3.5}, the ``inter-state'' average score skyrockets by near 9 absolute points from the standard setting. A similar leap of near 7 absolute points is seen in InternVL3.5-4B-Instruct~\cite{InternVL3.5}. The gains in inter-state \textbf{attribute recognition} and \textbf{reasoning} are particularly notable. This strongly suggests that the hierarchical approach, by forcing the model to explicitly serialize the timeline of events into a textual narrative, effectively mitigates the tendency of end-to-end models to overlook or conflate subtle temporal changes, leading to a far superior understanding of state transitions.

\noindent\textbf{Isolating the Inter-State Defect.}
% The most pronounced performance gaps are observed in the \textbf{``inter-state''} evaluation, which forms the core comparative challenge of our benchmark. As shown in (Fig~\ref{fig:inter}), for InternVL3.5-8B-Instruct~\cite{InternVL3.5}, a massive portion of previously incorrect predictions transition to correct ones under the text-oracle setting, causing the inter-state average score to skyrocket by nearly 9 absolute points. The improvements in inter-state \textbf{attribute recognition} and \textbf{reasoning} are particularly notable. This strongly suggests that forcing the explicit serialization of temporal events into text mitigates the severe tendency of current end-to-end vision-language projectors to overlook, overwrite, or conflate subtle temporal changes across disconnected states.
The most pronounced performance discrepancies between the standard baseline and the text-oracle probe are observed in the \textbf{`inter-state'} evaluation, which represents the core comparative challenge of our benchmark. As shown in Fig~\ref{fig:inter}, for InternVL3.5-8B-Instruct~\cite{InternVL3.5}, a massive portion of initially incorrect predictions are successfully converted to correct answers under the text-oracle setting, causing the ``inter-state'' average score to skyrocket by nearly 9 absolute points. A similar leap of nearly 7 absolute points is observed for InternVL3.5-4B-Instruct~\cite{InternVL3.5}. This dramatic shift reveals a critical vulnerability: while the models possess the requisite reasoning capacity, their standard end-to-end vision-language projectors struggle severely to maintain, track, and contrast subtle temporal changes across disconnected video states. By forcing the model to explicitly serialize the timeline of events into a textual narrative, the text-oracle effectively mitigates this tendency to overlook or conflate cross-state information.

\begin{figure}[h]
  \centering
    \centerline{\includegraphics[width=0.97\columnwidth]{imgs/baselines.pdf}}
    \caption{Performance comparison of experimental performance between LMM and LLM. ``Base'' refers to the results from the end-to-end model. ``HCTR'' denotes the results of performing HCTR using only the LMM. ``HCTR+Qwen'' represents the results of using the Qwen3~\cite{qwen3} to summarize clip captions and answer the question.}
    \label{fig:baseline_LLM}
\end{figure}

\noindent\textbf{Further Probe: LMM vs. Pure LLM for Textual Reasoning}
% We also explore a hybrid approach using text-only LLMs~\cite{qwen3} to summarize clip captions and answer the question. As shown in~\ref{fig:baseline_LLM}, our findings reveal a clear trend: when using an LLM of a comparable size to the LMM's language backbone, this hybrid approach outperforms the original end-to-end basemodel results but falls short of the full LMM pipeline. Notably, however, as we employ progressively larger and more powerful LLMs for the reasoning component, the performance of the hybrid system steadily increases, eventually exceeding that of the integrated LMM pipeline. This outcome yields two critical insights:
% \begin{enumerate}
%     \item The integrated visual grounding within the full LMM pipeline offers a tangible advantage, likely by preserving a richer, more contextually-aware representation through the intermediate stages. This is evidenced by its superior performance over the hybrid model when the language components are of comparable size.
    
%     \item The ultimate performance is heavily contingent on the power of the reasoning module. The fact that a superior reasoning-focused LLM can compensate for and ultimately surpass the architecturally integrated LMM pipeline underscores that advanced reasoning capability is a paramount, and potentially overriding, factor for success in complex multimodal tasks.
% \end{enumerate}
To push our diagnosis further, we explored replacing the reasoning component of the Text-Oracle with external, text-only LLMs~\cite{qwen3}. As shown in Fig~\ref{fig:baseline_LLM}, our findings reveal a clear scaling trend: when using an external LLM of a comparable size to the LMM's language backbone, the decoupled system falls short of the integrated LMM operating in Text-Oracle mode. However, as we substitute progressively larger and more powerful text-only LLMs (e.g., 32B), the performance of the decoupled system steadily increases, eventually exceeding the limits of the integrated LMM. This diagnostic outcome yields two critical insights:
\begin{enumerate}
    \item \textbf{The value of integrated training:} The integrated LMM (when given text-oracle context) still outperforms a blindly decoupled LLM of similar size. This indicates that joint multimodal training preserves a richer, more contextually-aware representation even when reasoning is forced through text intermediate stages.
    
    \item \textbf{Reasoning ceiling dictates the upper bound:} The ultimate performance on this comparative task is heavily contingent on pure logical capacity. The fact that a massively scaled reasoning-focused LLM can compensate for and ultimately surpass the native LMM pipeline underscores that while visual alignment is the current primary bottleneck, advancing pure logical reasoning capability remains a paramount prerequisite for success in complex spatial-temporal tasks.
\end{enumerate}

==> tabs/Qwen3_exp.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.08}
\small
% \footnotesize
\caption{Performance of various models on \textbf{\simsubset}. S. U. = Spatial Understanding, T. U. = Temporal Understanding, A. R. = Attribute Recognition, Rs = Reasoning. By default, models are evaluated with \textbf{200 input frames per video} at a resolution of \textbf{448$\times$448}, with thinking mode shut off. Models marked with \textsuperscript{*} use only 60 frames, and the model marked with \textsuperscript{\dag} employs an input resolution of 336$\times$448.}
% \caption{Performance of various vision–language models on \textbf{\simsubset}. Darker shades indicate better performance. By default, models are evaluated with \textbf{200 input frames per video} at a resolution of \textbf{448$\times$448}, with thinking mode shut off. Models marked with \textsuperscript{*} use only 60 frames, and the model marked with \textsuperscript{\dag} employs an input resolution of 336$\times$448.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|ccccc|ccccc}
\toprule
   &
   &
   &
  \multicolumn{5}{c|}{\textbf{Intra-state}} &
  \multicolumn{5}{c}{\textbf{Inter-state}} \\   \cmidrule(lr){4-8} \cmidrule(lr){9-13}
  \multirow{-2}{*}{\textbf{Model}} &
  \multirow{-2}{*}{\textbf{Size}} &
  \multirow{-2}{*}{\textbf{Overall}} &
  \textbf{Avg.} &
  \textbf{S. U.} &
  \textbf{T. U.} &
  \textbf{A. R.} &
  \multicolumn{1}{c|}{\textbf{Rs}} &
  \textbf{Avg.} &
  \textbf{S. U.} &
  \textbf{T. U.} &
  \textbf{A. R.} &
  \textbf{Rs} \\ \midrule
\multirow{6}{*}{Qwen3\cite{qwen3}} 
&  0.6B & 20.42  & 22.09  & 22.29 & 26.80  & 21.80 & 21.67 & 19.15  & 20.24  & 19.45 & 20.19 & 14.46  \\
& 1.4B & 24.45 & 23.915 & 27.43  & 27.24  & 25.995 & 18.89 & 24.93 & 27.59  & 23.47  & 22.39 & 26.93  \\
& 4B   & 28.78 & 31.04  & 30.78  & 26.295 & 33.57  & 32.91 & 26.74 & 30.235 & 26.26 & 23.54  & 26.8   \\
& 8B   & 32.22  & 32.60 & 29.72  & 35.82  & 33.66 & 38.35 & 32.395 & 32.43  & 30.98  & 30.68 & 38.40 \\
& 14B  & 34.37  & 33.15  & 33.33  & 38.52 & 33.06  & 34.83 & 34.79  & 36.99  & 33.83 & 33.38 & 37.24  \\
& 32B  & 32.97 & 34.37 & 33.92  & 41.66  & 34.58 & 36.52  & 30.82  & 34.62 & 29.43  & 29.21 & 30.75 \\
 \bottomrule
\end{tabular}
}
\label{tab:text-only-LLM_exp}
\end{table*}

==> tabs/basemodel_exp_real.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.08}
\small
% \footnotesize
\caption{Performance of various models on \textbf{\realsubset}.}

\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|c|cccc|c|cccc}
\toprule
   &
   &
   &
  \multicolumn{5}{c|}{\textbf{Intra-state}} &
  \multicolumn{5}{c}{\textbf{Inter-state}} \\   \cmidrule(lr){4-8} \cmidrule(lr){9-13}
  \multirow{-2}{*}{\textbf{Model}} &
  \multirow{-2}{*}{\textbf{Size}} &
  \multirow{-2}{*}{\textbf{Overall}} &
  \textbf{Avg.} &
  \textbf{S. U.} &
  \textbf{T. U.} &
  \textbf{A. R.} &
  \multicolumn{1}{c|}{\textbf{Rs}} &
  \textbf{Avg.} &
  \textbf{S. U.} &
  \textbf{T. U.} &
  \textbf{A. R.} &
  \textbf{Rs} \\ \midrule
\multicolumn{13}{l}{\textit{Proprietary LMMs}} \\ 
  Gemini-2.5-pro &
  -- &
  \cellcolor[HTML]{83C1B5}58.95 &
  \cellcolor[HTML]{72B8AB}69.73 &
  \cellcolor[HTML]{70B8AA}70.76 &
  \cellcolor[HTML]{8BC5BA}54.55 &
  \cellcolor[HTML]{6FB7A9}71.43 &
  \cellcolor[HTML]{75BAAC}68.00 &
  \cellcolor[HTML]{97CBC1}47.27 &
  \cellcolor[HTML]{90C8BD}51.02 &
  \cellcolor[HTML]{95CAC0}48.25 &
  \cellcolor[HTML]{98CCC2}46.41 &
  \cellcolor[HTML]{A5D2C9}38.75 \\ \midrule
\multicolumn{13}{l}{\textit{Open-Source LMMs}} \\ 
  WeThink-VL-7B~\cite{WeThink} &
  7B &
  \cellcolor[HTML]{BDDFD8}23.81 &
  \cellcolor[HTML]{B8DCD5}26.99 &
  \cellcolor[HTML]{BCDED8}24.56 &
  \cellcolor[HTML]{C6E4DE}18.18 &
  \cellcolor[HTML]{B5DBD4}28.57 &
  \cellcolor[HTML]{B3DAD2}30.00 &
  \cellcolor[HTML]{C4E2DC}19.85 &
  \cellcolor[HTML]{C4E3DD}19.27 &
  \cellcolor[HTML]{C5E3DD}19.25 &
  \cellcolor[HTML]{C5E3DD}18.78 &
  \cellcolor[HTML]{BCDED7}24.69 \\
  Video-R1-7B~\cite{Video-R1} &
  7B &
  \cellcolor[HTML]{A5D3CA}38.22 &
  \cellcolor[HTML]{A3D2C9}39.47 &
  \cellcolor[HTML]{A3D2C9}39.47 &
  \cellcolor[HTML]{9ACDC3}45.45 &
  \cellcolor[HTML]{A7D4CB}36.99 &
  \cellcolor[HTML]{9ECFC5}43.00 &
  \cellcolor[HTML]{A8D4CC}36.52 &
  \cellcolor[HTML]{A8D4CC}36.50 &
  \cellcolor[HTML]{A6D3CA}38.10 &
  \cellcolor[HTML]{ACD6CE}34.18 &
  \cellcolor[HTML]{A7D4CB}37.04 \\
  Video-XL-2~\cite{Video-XL-2} &
  8B &
  \cellcolor[HTML]{AAD5CD}35.13 &
  \cellcolor[HTML]{A2D1C8}40.46 &
  \cellcolor[HTML]{A1D1C7}40.74 &
  \cellcolor[HTML]{92C9BE}50.00 &
  \cellcolor[HTML]{A5D3CA}38.35 &
  \cellcolor[HTML]{9FD0C6}42.00 &
  \cellcolor[HTML]{B1D9D1}31.13 &
  \cellcolor[HTML]{B2D9D2}30.52 &
  \cellcolor[HTML]{AED7CF}32.98 &
  \cellcolor[HTML]{B3DAD2}29.75 &
  \cellcolor[HTML]{B2D9D2}30.25 \\
  MiniCPM-V-4.5~\cite{MiniCPM-V-4.5} &
  8B &
  \cellcolor[HTML]{A0D0C7}41.62 &
  \cellcolor[HTML]{8FC8BD}51.60 &
  \cellcolor[HTML]{8EC7BC}52.44 &
  \cellcolor[HTML]{74BAAC}68.18 &
  \cellcolor[HTML]{92C9BE}49.83 &
  \cellcolor[HTML]{92C9BE}50.00 &
  \cellcolor[HTML]{AFD8D0}32.33 &
  \cellcolor[HTML]{B3DAD2}30.01 &
  \cellcolor[HTML]{A8D4CC}36.71 &
  \cellcolor[HTML]{B1D9D1}30.91 &
  \cellcolor[HTML]{B6DBD4}28.40 \\
  InternVideo2.5-8B\textsuperscript{*}~\cite{InternVideo2.5} &
  8B &
  \cellcolor[HTML]{A7D4CB}37.03 &
  \cellcolor[HTML]{94CAC0}48.64 &
  \cellcolor[HTML]{91C9BE}50.39 &
  \cellcolor[HTML]{92C9BE}50.00 &
  \cellcolor[HTML]{93CABF}49.32 &
  \cellcolor[HTML]{9CCEC4}44.00 &
  \cellcolor[HTML]{B9DDD6}26.08 &
  \cellcolor[HTML]{B6DCD4}27.81 &
  \cellcolor[HTML]{B7DCD5}27.26 &
  \cellcolor[HTML]{BBDED7}25.00 &
  \cellcolor[HTML]{C1E1DB}21.60 \\
  VideoLLaMA3-7B\textsuperscript{\dag,*}\cite{VideoLLaMA3} &
  7B &
  \cellcolor[HTML]{9FD0C6}42.09 &
  \cellcolor[HTML]{94CABF}48.86 &
  \cellcolor[HTML]{95CBC0}48.06 &
  \cellcolor[HTML]{87C3B8}56.52 &
  \cellcolor[HTML]{93C9BF}49.59 &
  \cellcolor[HTML]{97CBC1}47.06 &
  \cellcolor[HTML]{ABD6CD}34.87 &
  \cellcolor[HTML]{B3DAD2}29.71 &
  \cellcolor[HTML]{A4D2C9}38.97 &
  \cellcolor[HTML]{A5D3CA}38.23 &
  \cellcolor[HTML]{B6DBD4}28.31 \\
  LLaVA-OneVision-1.5-8B~\cite{Llava-OneVision-1.5} &
  8B &
  \cellcolor[HTML]{B8DCD5}26.99 &
  \cellcolor[HTML]{B0D8D0}31.77 &
  \cellcolor[HTML]{ACD6CE}34.31 &
  \cellcolor[HTML]{B0D8D0}31.82 &
  \cellcolor[HTML]{AED7CF}32.99 &
  \cellcolor[HTML]{BBDED7}25.00 &
  \cellcolor[HTML]{BEE0D9}22.94 &
  \cellcolor[HTML]{C6E3DE}18.40 &
  \cellcolor[HTML]{BCDED8}24.44 &
  \cellcolor[HTML]{B7DCD5}27.27 &
  \cellcolor[HTML]{C4E2DC}19.75 \\
  InternVL3.5-2B\textsuperscript{*}~\cite{InternVL3.5} &
  2B &
  \cellcolor[HTML]{A8D4CC}36.64 &
  \cellcolor[HTML]{9DCEC5}43.46 &
  \cellcolor[HTML]{9BCDC4}44.74 &
  \cellcolor[HTML]{92C9BE}50.00 &
  \cellcolor[HTML]{9FD0C6}41.84 &
  \cellcolor[HTML]{9ECFC5}43.00 &
  \cellcolor[HTML]{B3D9D2}30.23 &
  \cellcolor[HTML]{ADD7CF}33.59 &
  \cellcolor[HTML]{B3DAD2}29.88 &
  \cellcolor[HTML]{BADDD7}25.63 &
  \cellcolor[HTML]{ADD7CF}33.33 \\
  InternVL3.5-4B\textsuperscript{*}~\cite{InternVL3.5} &
  4B &
  \cellcolor[HTML]{A7D4CB}36.96 &
  \cellcolor[HTML]{A0D0C6}41.82 &
  \cellcolor[HTML]{A3D1C8}39.77 &
  \cellcolor[HTML]{A8D4CC}36.36 &
  \cellcolor[HTML]{A0D0C7}41.58 &
  \cellcolor[HTML]{97CBC1}47.00 &
  \cellcolor[HTML]{B1D9D1}31.00 &
  \cellcolor[HTML]{B0D8D0}31.90 &
  \cellcolor[HTML]{B1D9D1}30.95 &
  \cellcolor[HTML]{B2D9D2}30.54 &
  \cellcolor[HTML]{B2D9D2}30.25 \\
  InternVL3.5-8B\textsuperscript{*}~\cite{InternVL3.5} &
  8B &
  \cellcolor[HTML]{A5D2CA}38.60 &
  \cellcolor[HTML]{91C9BE}50.51 &
  \cellcolor[HTML]{92C9BE}50.29 &
  \cellcolor[HTML]{B0D8D0}31.82 &
  \cellcolor[HTML]{92C9BE}50.00 &
  \cellcolor[HTML]{88C4B8}56.00 &
  \cellcolor[HTML]{B5DBD4}28.57 &
  \cellcolor[HTML]{B7DCD5}27.25 &
  \cellcolor[HTML]{AFD8D0}32.42 &
  \cellcolor[HTML]{B9DDD6}26.16 &
  \cellcolor[HTML]{BADDD6}25.93 \\
  Qwen3-VL-2B~\cite{qwen3-vl} &
  2B &
  \cellcolor[HTML]{A5D3CA}38.44 &
  \cellcolor[HTML]{92C9BE}50.31 &
  \cellcolor[HTML]{8BC5BA}54.39 &
  \cellcolor[HTML]{92C9BE}50.00 &
  \cellcolor[HTML]{9ACDC3}45.41 &
  \cellcolor[HTML]{8DC6BB}53.00 &
  \cellcolor[HTML]{B7DCD5}27.29 &
  \cellcolor[HTML]{B9DDD6}26.48 &
  \cellcolor[HTML]{B7DCD5}27.22 &
  \cellcolor[HTML]{BBDED7}25.11 &
  \cellcolor[HTML]{ADD7CF}33.33 \\
  Qwen3-VL-4B~\cite{qwen3-vl} &
  4B &
  \cellcolor[HTML]{A4D2C9}38.80 &
  \cellcolor[HTML]{99CDC3}45.60 &
  \cellcolor[HTML]{91C8BE}50.58 &
  \cellcolor[HTML]{A8D4CC}36.36 &
  \cellcolor[HTML]{9ACDC3}45.15 &
  \cellcolor[HTML]{A3D1C8}40.00 &
  \cellcolor[HTML]{B4DAD3}29.17 &
  \cellcolor[HTML]{B3DAD2}30.01 &
  \cellcolor[HTML]{B1D9D1}31.27 &
  \cellcolor[HTML]{B7DCD5}27.48 &
  \cellcolor[HTML]{BBDED7}25.31 \\
  Qwen3-VL-8B~\cite{qwen3-vl} &
  8B &
  \cellcolor[HTML]{9FCFC6}42.26 &
  \cellcolor[HTML]{8DC6BB}53.17 &
  \cellcolor[HTML]{8EC7BC}52.63 &
  \cellcolor[HTML]{9ACDC3}45.45 &
  \cellcolor[HTML]{8CC6BB}53.57 &
  \cellcolor[HTML]{8AC5B9}55.00 &
  \cellcolor[HTML]{B2D9D2}30.39 &
  \cellcolor[HTML]{B9DDD6}26.53 &
  \cellcolor[HTML]{AED7CF}32.74 &
  \cellcolor[HTML]{B1D9D1}31.33 &
  \cellcolor[HTML]{B2D9D2}30.25 \\ \bottomrule
\end{tabular}
}
\label{tab:real_basemodel_exp}
\end{table*}

==> tabs/basemodel_exp_sim.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.08}
\small
% \footnotesize
\caption{Performance of various models on \textbf{\simsubset}.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|c|cccc|c|cccc}
\toprule
   &
   &
   &
  \multicolumn{5}{c|}{\textbf{Intra-state}} &
  \multicolumn{5}{c}{\textbf{Inter-state}} \\   \cmidrule(lr){4-8} \cmidrule(lr){9-13}
  \multirow{-2}{*}{\textbf{Model}} &
  \multirow{-2}{*}{\textbf{Size}} &
  \multirow{-2}{*}{\textbf{Overall}} &
  \textbf{Avg.} &
  \textbf{S. U.} &
  \textbf{T. U.} &
  \textbf{A. R.} &
  \multicolumn{1}{c|}{\textbf{Rs}} &
  \textbf{Avg.} &
  \textbf{S. U.} &
  \textbf{T. U.} &
  \textbf{A. R.} &
  \textbf{Rs} \\ \midrule
\multicolumn{13}{l}{\textit{Proprietary LMMs}} \\ 
  Gemini-2.5-pro &
  -- &
  \cellcolor[HTML]{A9D4CC}36.21 &
  \cellcolor[HTML]{A8D4CC}36.69 &
  \cellcolor[HTML]{A2D1C8}40.02 &
  \cellcolor[HTML]{ABD6CD}34.75 &
  \cellcolor[HTML]{9ACDC3}45.07 &
  \cellcolor[HTML]{B3DAD3}29.65 &
  \cellcolor[HTML]{A8D4CC}36.38 &
  \cellcolor[HTML]{A4D2C9}38.79 &
  \cellcolor[HTML]{A9D5CC}35.81 &
  \cellcolor[HTML]{A0D0C7}41.35 &
  \cellcolor[HTML]{ADD7CF}33.41 \\
  GPT-5 &
  -- &
  \cellcolor[HTML]{9ACDC3}45.14 &
  \cellcolor[HTML]{9ACDC3}45.20 &
  \cellcolor[HTML]{97CCC1}46.82 &
  \cellcolor[HTML]{98CCC2}46.58 &
  \cellcolor[HTML]{90C8BD}51.20 &
  \cellcolor[HTML]{A5D3CA}38.27 &
  \cellcolor[HTML]{9ACDC3}45.29 &
  \cellcolor[HTML]{97CCC1}46.81 &
  \cellcolor[HTML]{98CCC2}46.65 &
  \cellcolor[HTML]{98CCC2}46.51 &
  \cellcolor[HTML]{9FCFC6}42.37 \\ \midrule
\multicolumn{13}{l}{\textit{Open-Source LMMs}} \\ 
  WeThink-VL-7B~\cite{WeThink} &
  7B &
  \cellcolor[HTML]{C6E4DE}18.24 &
  \cellcolor[HTML]{CAE5E0}16.19 &
  \cellcolor[HTML]{C8E4DF}17.21 &
  \cellcolor[HTML]{CCE7E1}14.59 &
  \cellcolor[HTML]{C3E2DC}20.25 &
  \cellcolor[HTML]{CDE7E2}14.07 &
  \cellcolor[HTML]{C0E1DA}21.75 &
  \cellcolor[HTML]{BADDD6}25.90 &
  \cellcolor[HTML]{C1E1DB}21.17 &
  \cellcolor[HTML]{C1E1DB}21.55 &
  \cellcolor[HTML]{C3E2DC}19.96 \\
  Video-R1-7B~\cite{Video-R1} &
  7B &
  \cellcolor[HTML]{B5DBD4}28.58 &
  \cellcolor[HTML]{B5DBD3}28.93 &
  \cellcolor[HTML]{B2D9D2}30.32 &
  \cellcolor[HTML]{B3DAD2}29.97 &
  \cellcolor[HTML]{B0D8D0}31.82 &
  \cellcolor[HTML]{BCDED8}24.58 &
  \cellcolor[HTML]{B4DAD3}29.47 &
  \cellcolor[HTML]{B1D9D1}30.94 &
  \cellcolor[HTML]{B4DAD3}29.58 &
  \cellcolor[HTML]{B6DBD4}27.97 &
  \cellcolor[HTML]{B4DAD3}29.10 \\
  Video-XL-2~\cite{Video-XL-2} &
  8B &
  \cellcolor[HTML]{B2D9D2}30.59 &
  \cellcolor[HTML]{B5DBD4}28.53 &
  \cellcolor[HTML]{B4DAD3}29.40 &
  \cellcolor[HTML]{B4DAD3}29.58 &
  \cellcolor[HTML]{B3DAD2}30.02 &
  \cellcolor[HTML]{BADDD7}25.61 &
  \cellcolor[HTML]{AED7CF}33.06 &
  \cellcolor[HTML]{AAD5CD}35.38 &
  \cellcolor[HTML]{AFD7D0}32.63 &
  \cellcolor[HTML]{B2D9D1}30.71 &
  \cellcolor[HTML]{AED7CF}33.16 \\
  MiniCPM-V-4.5~\cite{MiniCPM-V-4.5} &
  8B &
  \cellcolor[HTML]{B0D8D1}31.68 &
  \cellcolor[HTML]{B2D9D2}30.42 &
  \cellcolor[HTML]{B2D9D2}30.30 &
  \cellcolor[HTML]{AED7CF}32.89 &
  \cellcolor[HTML]{B1D9D1}31.25 &
  \cellcolor[HTML]{B7DCD5}27.61 &
  \cellcolor[HTML]{ADD6CE}33.80 &
  \cellcolor[HTML]{ACD6CE}34.33 &
  \cellcolor[HTML]{ABD6CD}34.75 &
  \cellcolor[HTML]{B1D9D1}31.28 &
  \cellcolor[HTML]{ADD7CF}33.53 \\
  InternVideo2.5-8B\textsuperscript{*}~\cite{InternVideo2.5} &
  8B &
  \cellcolor[HTML]{ADD7CF}33.30 &
  \cellcolor[HTML]{AFD8D0}32.56 &
  \cellcolor[HTML]{ACD6CE}34.18 &
  \cellcolor[HTML]{AED7CF}32.76 &
  \cellcolor[HTML]{A7D3CB}37.49 &
  \cellcolor[HTML]{B7DCD5}27.48 &
  \cellcolor[HTML]{ABD5CD}35.06 &
  \cellcolor[HTML]{AAD5CD}35.14 &
  \cellcolor[HTML]{ABD6CE}34.56 &
  \cellcolor[HTML]{A7D4CB}37.23 &
  \cellcolor[HTML]{ABD6CE}34.62 \\
  VideoLLaMA3-7B\textsuperscript{\dag,*}\cite{VideoLLaMA3} &
  7B &
  \cellcolor[HTML]{A9D5CC}35.87 &
  \cellcolor[HTML]{ADD7CF}33.55 &
  \cellcolor[HTML]{ADD7CF}33.37 &
  \cellcolor[HTML]{AAD5CD}35.26 &
  \cellcolor[HTML]{A7D4CB}37.13 &
  \cellcolor[HTML]{B3DAD2}29.81 &
  \cellcolor[HTML]{A4D2C9}39.39 &
  \cellcolor[HTML]{A1D0C7}41.20 &
  \cellcolor[HTML]{A7D4CB}37.26 &
  \cellcolor[HTML]{9ECFC5}42.82 &
  \cellcolor[HTML]{A4D2C9}39.13 \\
  LLaVA-OneVision-1.5-8B~\cite{Llava-OneVision-1.5} &
  8B &
  \cellcolor[HTML]{AED7CF}32.83 &
  \cellcolor[HTML]{B6DBD4}28.02 &
  \cellcolor[HTML]{B5DBD3}28.74 &
  \cellcolor[HTML]{B7DCD4}27.67 &
  \cellcolor[HTML]{B3DAD2}30.07 &
  \cellcolor[HTML]{B9DDD6}26.28 &
  \cellcolor[HTML]{A7D4CB}37.17 &
  \cellcolor[HTML]{ACD6CE}34.29 &
  \cellcolor[HTML]{A8D4CB}36.73 &
  \cellcolor[HTML]{9DCEC5}43.37 &
  \cellcolor[HTML]{A8D4CB}36.72 \\
  InternVL3.5-2B\textsuperscript{*}~\cite{InternVL3.5} &
  2B &
  \cellcolor[HTML]{AED7CF}32.80 &
  \cellcolor[HTML]{BADDD6}25.74 &
  \cellcolor[HTML]{B7DCD4}27.70 &
  \cellcolor[HTML]{BBDED7}25.06 &
  \cellcolor[HTML]{BADDD6}25.90 &
  \cellcolor[HTML]{BCDFD8}24.18 &
  \cellcolor[HTML]{A1D1C8}40.73 &
  \cellcolor[HTML]{A2D1C8}40.22 &
  \cellcolor[HTML]{A8D4CC}36.53 &
  \cellcolor[HTML]{8FC8BD}51.71 &
  \cellcolor[HTML]{A1D1C7}40.86 \\
  InternVL3.5-4B\textsuperscript{*}~\cite{InternVL3.5} &
  4B &
  \cellcolor[HTML]{AAD5CD}35.47 &
  \cellcolor[HTML]{AFD7D0}32.63 &
  \cellcolor[HTML]{AED7CF}32.99 &
  \cellcolor[HTML]{ADD7CF}33.39 &
  \cellcolor[HTML]{ACD6CE}34.17 &
  \cellcolor[HTML]{B2D9D2}30.52 &
  \cellcolor[HTML]{A5D3CA}38.46 &
  \cellcolor[HTML]{A3D1C8}39.78 &
  \cellcolor[HTML]{ABD6CE}34.62 &
  \cellcolor[HTML]{99CDC3}45.51 &
  \cellcolor[HTML]{A5D2C9}38.78 \\
  InternVL3.5-8B\textsuperscript{*}~\cite{InternVL3.5} &
  8B &
  \cellcolor[HTML]{B1D9D1}31.04 &
  \cellcolor[HTML]{B1D9D1}31.01 &
  \cellcolor[HTML]{B1D9D1}31.35 &
  \cellcolor[HTML]{AED7CF}33.20 &
  \cellcolor[HTML]{B0D8D0}31.86 &
  \cellcolor[HTML]{B6DBD4}27.97 &
  \cellcolor[HTML]{AED7CF}32.81 &
  \cellcolor[HTML]{AFD8D0}32.47 &
  \cellcolor[HTML]{ACD6CE}33.93 &
  \cellcolor[HTML]{B0D8D0}32.01 &
  \cellcolor[HTML]{AFD8D0}32.14 \\
  Qwen3-VL-2B~\cite{qwen3-vl} &
  2B &
  \cellcolor[HTML]{B1D9D1}31.35 &
  \cellcolor[HTML]{B4DAD3}29.56 &
  \cellcolor[HTML]{B2D9D1}30.78 &
  \cellcolor[HTML]{B1D9D1}31.24 &
  \cellcolor[HTML]{B1D9D1}30.99 &
  \cellcolor[HTML]{BADDD6}25.70 &
  \cellcolor[HTML]{ADD6CE}33.85 &
  \cellcolor[HTML]{ABD6CD}34.73 &
  \cellcolor[HTML]{B0D8D0}31.85 &
  \cellcolor[HTML]{A8D4CC}36.52 &
  \cellcolor[HTML]{ACD6CE}34.34 \\
  Qwen3-VL-4B~\cite{qwen3-vl} &
  4B &
  \cellcolor[HTML]{A5D2C9}38.78 &
  \cellcolor[HTML]{AAD5CD}35.51 &
  \cellcolor[HTML]{AAD5CD}35.21 &
  \cellcolor[HTML]{A4D2C9}39.04 &
  \cellcolor[HTML]{A5D3CA}38.29 &
  \cellcolor[HTML]{B2D9D2}30.64 &
  \cellcolor[HTML]{9FD0C6}41.99 &
  \cellcolor[HTML]{A0D0C7}41.54 &
  \cellcolor[HTML]{A2D1C8}40.20 &
  \cellcolor[HTML]{8FC7BC}52.17 &
  \cellcolor[HTML]{A3D1C8}39.81 \\
  Qwen3-VL-8B~\cite{qwen3-vl} &
  8B &
  \cellcolor[HTML]{A9D5CC}35.87 &
  \cellcolor[HTML]{A9D5CC}35.82 &
  \cellcolor[HTML]{AED7CF}33.29 &
  \cellcolor[HTML]{A5D3CA}38.56 &
  \cellcolor[HTML]{A1D1C7}40.82 &
  \cellcolor[HTML]{AED7CF}32.71 &
  \cellcolor[HTML]{A7D3CB}37.46 &
  \cellcolor[HTML]{A2D1C8}40.06 &
  \cellcolor[HTML]{A6D3CA}37.77 &
  \cellcolor[HTML]{A9D4CC}36.33 &
  \cellcolor[HTML]{A9D5CC}36.05 \\
  Qwen3-VL-235B-A22B~\cite{qwen3-vl} &
  235B &
  \cellcolor[HTML]{A5D2CA}38.60 &
  \cellcolor[HTML]{A8D4CC}36.46 &
  \cellcolor[HTML]{A6D3CA}37.74 &
  \cellcolor[HTML]{A6D3CA}37.88 &
  \cellcolor[HTML]{A4D2C9}39.38 &
  \cellcolor[HTML]{B0D8D0}31.82 &
  \cellcolor[HTML]{A1D0C7}41.13 &
  \cellcolor[HTML]{A3D2C9}39.40 &
  \cellcolor[HTML]{A3D1C8}39.92 &
  \cellcolor[HTML]{9ACDC3}44.93 &
  \cellcolor[HTML]{9FD0C6}41.85 \\ \bottomrule
\end{tabular}
}
\label{tab:sim_basemodel_exp}
\end{table*}

==> tabs/correlation.tex <==
\begin{table}[htbp]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt} 
\renewcommand{\arraystretch}{0.3}
\setlength{\abovecaptionskip}{-1pt}
\setlength{\belowcaptionskip}{-3pt}
\caption{\textbf{Spearman Corre. with Other General Benchmarks}}
\label{tab:spearman_correlation}
\begin{tabular}{c*{5}{c}}
\toprule
\textbf{MVBench} & \textbf{VideoMME} & \textbf{MLVU} & \textbf{LVBench} & \textbf{CharadesSTA} & \textbf{VideoMMMU} \\
\cmidrule{1-6}
\textbf{0.37} &
  \textbf{0.70} &
  \textbf{0.70} &
  \textbf{0.61} &
  \textbf{0.64} &
  \textbf{0.71} \\
\bottomrule
\end{tabular}
\end{table}


==> tabs/hallucination.tex <==
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.08}
\scriptsize
\caption{Overall Accuracy comparison on hallucination  questions. Darker shades indicate  more severe hallucination issues. }
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|c|c|c}
\toprule
  \textbf{Model} &
  \textbf{Hall.} &
  \textbf{Fac.}&
  \textbf{Fac. - Hall.} \\ \midrule
    Gemini-2.5-pro          & 43.89     & 33.89  & \cellcolor[HTML]{FFFFFF}-10.00    \\
    GPT-5                   & 38.44     & 47.16  & \cellcolor[HTML]{DCF0DA}8.72      \\
    \midrule
    WeThink-Qwen2.5VL-7B~\cite{WeThink}    & 26.66     & 15.70  & \cellcolor[HTML]{FFFFFF}-10.96    \\
    InternVL3.5-2B~\cite{InternVL3.5} & 39.47     & 30.79  & \cellcolor[HTML]{FFFFFF}-8.68     \\
    InternVL3.5-4B~\cite{InternVL3.5} & 39.76     & 34.18  & \cellcolor[HTML]{FFFFFF}-5.58     \\
    Qwen3-VL-4B~\cite{qwen3-vl}    & 33.43     & 40.39  & \cellcolor[HTML]{E3F3E2}6.96      \\
    LLaVA-OneVision-1.5-8B~\cite{Llava-OneVision-1.5}  & 26.51     & 34.73  & \cellcolor[HTML]{DEF1DC}8.22      \\
    Qwen3-VL-2B~\cite{qwen3-vl}    & 22.83     & 33.92  & \cellcolor[HTML]{D3ECD0}11.09     \\
    VideoLLaMA3-7B~\cite{VideoLLaMA3}          & 23.71     & 39.54  & \cellcolor[HTML]{C0E4BC}15.83     \\
    Video-XL-2~\cite{Video-XL-2}              & 17.97     & 34.39  & \cellcolor[HTML]{BEE3BA}16.42     \\
    Qwen3-VL-235B~\cite{qwen3-vl}           & 24.15     & 42.96  & \cellcolor[HTML]{B5DFB0}18.81     \\
    Qwen3-VL-8B~\cite{qwen3-vl}    & 17.67     & 41.35  & \cellcolor[HTML]{A1D69C}23.68     \\
    Video-R1-7B~\cite{Video-R1}             & 7.51      & 34.93  & \cellcolor[HTML]{92D08C}27.42     \\
    InternVideo2.5-8B~\cite{InternVideo2.5}       & 11.49     & 39.87  & \cellcolor[HTML]{8FCE88}28.38     \\
    MiniCPM-V-4.5~\cite{MiniCPM-V-4.5}           & 8.84      & 38.57  & \cellcolor[HTML]{89CC82}29.73     \\
    InternVL3.5-8B~\cite{InternVL3.5} & 2.50      & 39.63  & \cellcolor[HTML]{6CBF63}37.13     \\
  \midrule
  \rowcolor{gray!10}
  \textbf{Average} & 24.05 & 36.38 & \cellcolor[HTML]{CEEACB}12.32\\
\bottomrule
\end{tabular}
}
\label{tab:hallucination}
\end{table}

==> tabs/hallucination_and_frame_sample.tex <==
\begin{figure}[tbp]
    \begin{minipage}[t]{0.46\linewidth}
        \centering
        \captionsetup{type=table, aboveskip=0pt}
        \caption{\textbf{Accuracy on hallucination questions.} Darker shades indicate more severe hallucination issues.}
        \label{tab:hallucination}

        \resizebox{\linewidth}{!}{%
            \begin{tabular}{l|c|c|c}
            \toprule
              \textbf{Model} &
              \textbf{Hall.} &
              \textbf{Fac.}&
              \textbf{Fac. - Hall.} \\ \midrule
                Gemini-2.5-pro          & 43.89     & 33.89  & \cellcolor[HTML]{FFFFFF}-10.00    \\
                GPT-5                   & 38.44     & 47.16  & \cellcolor[HTML]{DCF0DA}8.72      \\
                \midrule
                WeThink-Qwen2.5VL-7B~\cite{WeThink}    & 26.66     & 15.70  & \cellcolor[HTML]{FFFFFF}-10.96    \\
                InternVL3.5-2B~\cite{InternVL3.5} & 39.47     & 30.79  & \cellcolor[HTML]{FFFFFF}-8.68     \\
                InternVL3.5-4B~\cite{InternVL3.5} & 39.76     & 34.18  & \cellcolor[HTML]{FFFFFF}-5.58     \\
                Qwen3-VL-4B~\cite{qwen3-vl}    & 33.43     & 40.39  & \cellcolor[HTML]{E3F3E2}6.96      \\
                LLaVA-OneVision-1.5-8B~\cite{Llava-OneVision-1.5}  & 26.51     & 34.73  & \cellcolor[HTML]{DEF1DC}8.22      \\
                Qwen3-VL-2B~\cite{qwen3-vl}    & 22.83     & 33.92  & \cellcolor[HTML]{D3ECD0}11.09     \\
                VideoLLaMA3-7B~\cite{VideoLLaMA3}          & 23.71     & 39.54  & \cellcolor[HTML]{C0E4BC}15.83     \\
                Video-XL-2~\cite{Video-XL-2}              & 17.97     & 34.39  & \cellcolor[HTML]{BEE3BA}16.42     \\
                Qwen3-VL-235B~\cite{qwen3-vl}           & 24.15     & 42.96  & \cellcolor[HTML]{B5DFB0}18.81     \\
                Qwen3-VL-8B~\cite{qwen3-vl}    & 17.67     & 41.35  & \cellcolor[HTML]{A1D69C}23.68     \\
                Video-R1-7B~\cite{Video-R1}             & 7.51      & 34.93  & \cellcolor[HTML]{92D08C}27.42     \\
                InternVideo2.5-8B~\cite{InternVideo2.5}       & 11.49     & 39.87  & \cellcolor[HTML]{8FCE88}28.38     \\
                MiniCPM-V-4.5~\cite{MiniCPM-V-4.5}           & 8.84      & 38.57  & \cellcolor[HTML]{89CC82}29.73     \\
                InternVL3.5-8B~\cite{InternVL3.5} & 2.50      & 39.63  & \cellcolor[HTML]{6CBF63}37.13     \\
              \midrule
              \rowcolor{gray!10}
              \textbf{Average} & 24.05 & 36.38 & \cellcolor[HTML]{CEEACB}12.32\\
            \bottomrule
            \end{tabular}%
        }
    \end{minipage}%
    \hfill
    % 右侧：图片区域
    \begin{minipage}[t]{0.52\linewidth}
        \centering
        \includegraphics[width=\linewidth]{imgs/frame_sample/combined.pdf}
        \caption{An analysis of the impact of the number of sampled video frames on overall score in \textbf{\simsubset}. The results are shown for two models: \textit{Left}: Qwen3-VL-4B~\cite{qwen3-vl} and \textit{Right}: Video-XL-2~\cite{Video-XL-2} . It presents an upward trend as the number of frames increases.}
        \label{fig:frame_sampling}
    \end{minipage}
\end{figure}

==> tabs/option_distribution.tex <==
% \begin{table}[htbp]
% \centering
% \footnotesize
% \renewcommand{\arraystretch}{0.5}
% % \setlength{\tabcolsep}{2pt}
% \setlength{\abovecaptionskip}{-1pt}
% \setlength{\belowcaptionskip}{-4pt}
% \caption{\textbf{\#Opt. for Intra- \& Inter-state Tasks}}
% \begin{tabular}{l|c*{5}{c}|c}
% \toprule
% \textbf{\#Opt.} &
%   \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{Avg. \#Opt.} \\
% \cmidrule{1-8}
% \textbf{Intra} &
%   {\cellcolor[HTML]{FCFCFF}1} & 
%   {\cellcolor[HTML]{EFF7F4}69} &
%   {\cellcolor[HTML]{A1D8B1}470} &
%   {\cellcolor[HTML]{9FD7AF}481} &
%   {\cellcolor[HTML]{B2DEBF}385} &
%   {\cellcolor[HTML]{FAFBFD}14} &
%   {\textbf{4.86}} \\
% \textbf{Inter} &
%   {\cellcolor[HTML]{DBEFE2}175} &
%   {\cellcolor[HTML]{FCFCFF}4} &
%   {\cellcolor[HTML]{63BE7B}790} &
%   {\cellcolor[HTML]{C8E7D2}273} &
%   {\cellcolor[HTML]{C8E7D2}270} &
%   {\cellcolor[HTML]{FCFCFF}0} &
%   {\textbf{4.30}}\\
% \bottomrule
% \end{tabular}
% \label{tab:state_option_dist}
% \end{table}

\begin{table}[htbp]
\caption{Distribution of Option Numbers for \textbf{Intra-State} and \textbf{Inter-state} Tasks}
\label{tab:state_option_dist}

\scriptsize % 统一缩小字体
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} l|cccccc|l|cccccc|l}
\toprule
\textbf{Subset} &
  \multicolumn{7}{c|}{\textbf{\simsubset}} &
  \multicolumn{7}{c}{\textbf{\realsubset}}  \\
\midrule
\textbf{\#Opt} &
  \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{Avg.} &
  \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{9} & \textbf{Avg.} \\ 
\midrule
\textbf{Intra-State} &
  \cellcolor[HTML]{FFFFFF}1 & \cellcolor[HTML]{F2F9F1}69 & \cellcolor[HTML]{A8D9A2}470 &
  \cellcolor[HTML]{A5D8A0}481 & \cellcolor[HTML]{B7E0B3}385 & \cellcolor[HTML]{FCFEFC}14 &
  \textbf{4.86} &
  \cellcolor[HTML]{FFFFFF}2 & \cellcolor[HTML]{D3ECD0}238 & \cellcolor[HTML]{FBFDFA}24 &
  \cellcolor[HTML]{FEFFFE}4 & \cellcolor[HTML]{FFFFFF}0 & \cellcolor[HTML]{FFFFFF}0 &
  \textbf{4.11} \\
\textbf{Inter-State} &
  \cellcolor[HTML]{DEF1DC}175 & \cellcolor[HTML]{FEFFFE}4 & \cellcolor[HTML]{6CBF63}790 &
  \cellcolor[HTML]{CCE9C9}273 & \cellcolor[HTML]{CDE9CA}270 & \cellcolor[HTML]{FFFFFF}0 &
  \textbf{4.3} &
  \cellcolor[HTML]{FFFFFF}1 & \cellcolor[HTML]{D7EED5}215 & \cellcolor[HTML]{F5FBF4}54 &
  \cellcolor[HTML]{FDFEFD}11 & \cellcolor[HTML]{FFFFFF}2 & \cellcolor[HTML]{FFFFFF}1 &
  \textbf{4.3} \\ 
\bottomrule
\end{tabular*}
\end{table}

==> tabs/prompts/get_capabilities_prompt.tex <==
\begin{figure}[t]
\noindent
\begin{minipage}{\linewidth}
    \fcolorbox{gray!50!black}{white}{%
        \begin{minipage}{\dimexpr\linewidth-2\fboxsep-2\fboxrule\relax}
            \colorbox{gray!10}{%
                \parbox{\dimexpr\linewidth-10pt\relax}{%
                    \bfseries\itshape\scriptsize 
                    Capability Classification Prompt
                }%
            }%
            \vskip 2pt 
            \hrule height 0.5pt 
            \vskip 2pt 
            \tiny 
            You are a capability classification assistant. Given a question and some options, you need to determine which capabilities of the model this question tests.\\
            Please select one or more of the most relevant capabilities from the following list: temporal understanding, spatial understanding, attribute recognition, reasoning.\\
            Here are the descriptions for each capability to help you make a better judgment:
            \begin{itemize}
                \item[--] \textbf{temporal understanding}: Involves understanding and reasoning about temporal sequences, durations, and changes across observations. This includes determining object appearance order (first/last seen), observation duration comparisons, temporal state changes (before/after comparisons), and understanding event sequences in multi-state scenarios.
                \item[--] \textbf{spatial understanding}: Involves comprehending spatial relationships, positions, and arrangements in the environment. This includes object location determination (on/under surfaces), distance estimation between objects, spatial proximity comparisons, room layout understanding, and object containment relationships.
                \item[--] \textbf{attribute recognition}: Involves identifying and comparing object properties and characteristics. This includes color identification, shape recognition, size comparisons, material properties, object states (open/closed, on/off, filled/empty), visual appearance attributes across different observations, and scenarios where options themselves describe attributes.
                \item[--] \textbf{reasoning}: Involves logical deduction, quantitative analysis, and complex inference tasks. This includes counting objects, comparing quantities, performing multi-step logical reasoning, identifying patterns, making comparisons across different observations, synthesizing multiple information sources to draw conclusions, and situations requiring comparisons between different options.
            \end{itemize}
            
            Question: \{question\}\\
            Options: \{options\}\\
            
            Please return the result in JSON format, for example: \{\{"capabilities": ["capability1", "capability2"]\}\}.
            \vskip 2pt 
        \end{minipage}%
    }
\end{minipage}
\caption{The prompt used for classifying the capabilities required to answer each question. We define four core capabilities: temporal understanding, spatial understanding, attribute recognition, and reasoning.}
\label{fig:capability_prompt}
\end{figure}

==> tabs/real_table.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.08}
\small
\caption{Performance of various models. Darker shades indicate better performance.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccccccccccc}
\toprule
\textbf{Model} & \textbf{Col 1} & \textbf{Col 2} & \textbf{Col 3} & \textbf{Col 4} & \textbf{Col 5} & \textbf{Col 6} & \textbf{Col 7} & \textbf{Col 8} & \textbf{Col 9} & \textbf{Col 10} \\ \midrule
Gemini-2.5-Pro & \cellcolor[HTML]{82C08A}0.5895 & \cellcolor[HTML]{73B97E}0.6973 & \cellcolor[HTML]{70B77B}0.7076 & \cellcolor[HTML]{96CA9D}0.5455 & \cellcolor[HTML]{6FB578}0.7143 & \cellcolor[HTML]{7BBF85}0.6800 & \cellcolor[HTML]{A3D0A9}0.4727 & \cellcolor[HTML]{9CCDA3}0.5102 & \cellcolor[HTML]{A4D1AA}0.4825 & \cellcolor[HTML]{AAD4AF}0.4641 & \cellcolor[HTML]{B5DBBB}0.3875 \\
InternVL3\_5-4B & \cellcolor[HTML]{B3DABB}0.3696 & \cellcolor[HTML]{A9D4AE}0.4182 & \cellcolor[HTML]{ADD6B2}0.3977 & \cellcolor[HTML]{B5DBBB}0.3636 & \cellcolor[HTML]{A9D4AE}0.4158 & \cellcolor[HTML]{9DCDA3}0.4700 & \cellcolor[HTML]{C9E4CE}0.3100 & \cellcolor[HTML]{C8E4CD}0.3190 & \cellcolor[HTML]{C9E4CE}0.3095 & \cellcolor[HTML]{CAE5CF}0.3054 & \cellcolor[HTML]{CAE5CF}0.3025 \\
InternVL3\_5-8B & \cellcolor[HTML]{B0D9B7}0.3860 & \cellcolor[HTML]{A5D2AA}0.5051 & \cellcolor[HTML]{A6D2AB}0.5029 & \cellcolor[HTML]{C1E1C7}0.3182 & \cellcolor[HTML]{BEE0C4}0.5000 & \cellcolor[HTML]{9FD0A6}0.5600 & \cellcolor[HTML]{CDE7D2}0.2857 & \cellcolor[HTML]{D0E9D5}0.2725 & \cellcolor[HTML]{C8E4CD}0.3242 & \cellcolor[HTML]{D1EAD7}0.2616 & \cellcolor[HTML]{D2EAD8}0.2593 \\
InternVideo2\_5-8B & \cellcolor[HTML]{B2D9B9}0.3703 & \cellcolor[HTML]{A7D3AC}0.4864 & \cellcolor[HTML]{A6D2AB}0.5039 & \cellcolor[HTML]{BEE0C4}0.5000 & \cellcolor[HTML]{BBDDC1}0.4932 & \cellcolor[HTML]{A9D4AE}0.4400 & \cellcolor[HTML]{D1EAD7}0.2608 & \cellcolor[HTML]{CFE8D4}0.2781 & \cellcolor[HTML]{D0E9D5}0.2726 & \cellcolor[HTML]{D3EBD9}0.2500 & \cellcolor[HTML]{D6EDDC}0.2160 \\
LLaVA-OneVision-1.5 & \cellcolor[HTML]{C9E4CE}0.2699 & \cellcolor[HTML]{C2E1C7}0.3177 & \cellcolor[HTML]{BEE0C4}0.3431 & \cellcolor[HTML]{C1E1C7}0.3182 & \cellcolor[HTML]{C2E1C7}0.3299 & \cellcolor[HTML]{D1EAD7}0.2500 & \cellcolor[HTML]{D5ECDA}0.2294 & \cellcolor[HTML]{D9EFDF}0.1840 & \cellcolor[HTML]{D3EBD9}0.2444 & \cellcolor[HTML]{D0E9D5}0.2727 & \cellcolor[HTML]{DAF0E0}0.1975 \\
MiniCPM-V-4.5 & \cellcolor[HTML]{A7D3AC}0.4162 & \cellcolor[HTML]{9CD0A2}0.5160 & \cellcolor[HTML]{9AD0A0}0.5244 & \cellcolor[HTML]{78BC81}0.6818 & \cellcolor[HTML]{A3D0A8}0.4983 & \cellcolor[HTML]{BEE0C4}0.5000 & \cellcolor[HTML]{C8E4CD}0.3233 & \cellcolor[HTML]{CAE5CF}0.3001 & \cellcolor[HTML]{C3E2C8}0.3671 & \cellcolor[HTML]{CBE6D0}0.3091 & \cellcolor[HTML]{CCE7D1}0.2840 \\
Qwen3-VL-4B & \cellcolor[HTML]{B0D9B7}0.3880 & \cellcolor[HTML]{B1D9B8}0.4560 & \cellcolor[HTML]{A6D2AB}0.5058 & \cellcolor[HTML]{B5DBBB}0.3636 & \cellcolor[HTML]{B2D9B8}0.4515 & \cellcolor[HTML]{C4E3C9}0.4000 & \cellcolor[HTML]{CAE5CF}0.2917 & \cellcolor[HTML]{CAE5CF}0.3001 & \cellcolor[HTML]{C6E3CB}0.3127 & \cellcolor[HTML]{CBE6D0}0.2748 & \cellcolor[HTML]{D2EAD8}0.2531 \\
Qwen3-VL-8B & \cellcolor[HTML]{ADD6B2}0.4226 & \cellcolor[HTML]{9AD0A0}0.5317 & \cellcolor[HTML]{9AD0A0}0.5263 & \cellcolor[HTML]{A9D4AE}0.4545 & \cellcolor[HTML]{9ED0A5}0.5357 & \cellcolor[HTML]{9AD0A0}0.5500 & \cellcolor[HTML]{C9E4CE}0.3039 & \cellcolor[HTML]{CDE7D2}0.2653 & \cellcolor[HTML]{C5E3CB}0.3274 & \cellcolor[HTML]{C9E4CE}0.3133 & \cellcolor[HTML]{CAE5CF}0.3025 \\
Video-R1-7B & \cellcolor[HTML]{B2D9B9}0.3822 & \cellcolor[HTML]{B0D9B7}0.3947 & \cellcolor[HTML]{B0D9B7}0.3947 & \cellcolor[HTML]{A9D4AE}0.4545 & \cellcolor[HTML]{B4DABB}0.3699 & \cellcolor[HTML]{BDDFC3}0.4300 & \cellcolor[HTML]{C5E3CB}0.3652 & \cellcolor[HTML]{C5E3CB}0.3650 & \cellcolor[HTML]{C2E1C7}0.3810 & \cellcolor[HTML]{C8E4CD}0.3418 & \cellcolor[HTML]{C8E4CD}0.3704 \\
Video-XL-2 & \cellcolor[HTML]{B9DDC0}0.3513 & \cellcolor[HTML]{ADD6B2}0.4046 & \cellcolor[HTML]{ACD6B1}0.4074 & \cellcolor[HTML]{BEE0C4}0.5000 & \cellcolor[HTML]{B3DAB9}0.3835 & \cellcolor[HTML]{C0E0C6}0.4200 & \cellcolor[HTML]{C9E4CE}0.3113 & \cellcolor[HTML]{CAE5CF}0.3052 & \cellcolor[HTML]{C3E2C8}0.3298 & \cellcolor[HTML]{CAE5CF}0.2975 & \cellcolor[HTML]{CAE5CF}0.3025 \\
VideoLLaMA3-7B & \cellcolor[HTML]{AEE6B4}0.4209 & \cellcolor[HTML]{A6D2AB}0.4886 & \cellcolor[HTML]{A8D3AC}0.4806 & \cellcolor[HTML]{9AD0A0}0.5652 & \cellcolor[HTML]{A3D0A8}0.4959 & \cellcolor[HTML]{B7DDBE}0.4706 & \cellcolor[HTML]{C3E2C8}0.3487 & \cellcolor[HTML]{CAE5CF}0.2971 & \cellcolor[HTML]{C3E2C8}0.3897 & \cellcolor[HTML]{C4E3C9}0.3823 & \cellcolor[HTML]{D1EAD7}0.2831 \\
WeThink-Qwen2.5VL & \cellcolor[HTML]{D0E9D5}0.2381 & \cellcolor[HTML]{D1EAD7}0.2699 & \cellcolor[HTML]{D0E9D5}0.2456 & \cellcolor[HTML]{D5ECDA}0.1818 & \cellcolor[HTML]{D1EAD7}0.2857 & \cellcolor[HTML]{D1EAD7}0.3000 & \cellcolor[HTML]{D5ECDA}0.1985 & \cellcolor[HTML]{D6EDDC}0.1927 & \cellcolor[HTML]{D6EDDC}0.1925 & \cellcolor[HTML]{D7EEDD}0.1878 & \cellcolor[HTML]{D0E9D5}0.2469 \\
\bottomrule
\end{tabular}
}
\label{tab:performance_chart}
\end{table*}
